OReole-FM: successes and challenges toward billion-parameter foundation models for high-resolution satellite imagery

While the pretraining of Foundation Models (FMs) for remote sensing (RS) imagery is on the rise, models remain restricted to a few hundred million parameters. Scaling models to billions of parameters has been shown to yield unprecedented benefits including emergent abilities, but requires data scaling and computing resources typically not available outside industry R&D labs. In this work, we pair high-performance computing resources including Frontier supercomputer, America's first exascale system, and high-resolution optical RS data to pretrain billion-scale FMs. Our study assesses performance of different pretrained variants of vision Transformers across image classification, semantic segmentation and object detection benchmarks, which highlight the importance of data scaling for effective model scaling. Moreover, we discuss construction of a novel TIU pretraining dataset, model initialization, with data and pretrained models intended for public release. By discussing technical challenges and details often lacking in the related literature, this work is intended to offer best practices to the geospatial community toward efficient training and benchmarking of larger FMs.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/removedblank4_experiments.tex <==
\section{\textsc{Quetzal-MR} Experiments}
\label{sec:experiments_mr}

% - Discuss scalability DGX vs Frontier?

% \todo[inline]{Discuss downstream tasks, evaluation protocols adopted for evaluation of such FMs, to motivate/justify the evaluation we opted for. Not sure if at the end this will be in Related Works or Methods/Experiments- Include: UCM, AID, NWPU; Potsdam, LoveDA; DIOR, FAIR1M}

% \subsection{\textsc{Quetzal-MR} evaluation}

Since a main desired capability of FMs is the ability to extract generalizable features that can be easily adapted for multiple downstream tasks, evaluation protocols are typically based on the concepts of fine-tuning and linear probing. Related works introducing FM models for RS data typically report evaluation on three main set of tasks: image classification, object detection, and semantic segmentation. There is, however, a wide variability on the datasets used for performance benchmarking. We summarize in Table \ref{tab:eval_sets} the datasets used by closely related works for evaluation of models pretrained on medium-to-high resolution optical overhead imagery, for each of these three types of tasks. Based on this compiled information we selected two datasets for each task type to compose the downstream evaluation scenarios of our \textsc{Quetzal-MR} model variants. Highlighted in bold in the corresponding table, these datasets are discussed in details in the paragraphs that follow. 

  % \makecell{Object \\ Detection} & \makecell{\textbf{Semantic \\ Segmentation}}
\begin{table}[h]
    \centering
    \caption{Summary of datasets used in related works for evaluation of downstream capabilities of pretrained models. Highlighted in \textbf{bold} are the datasets we selected for evaluation of our models.}
    \label{tab:eval_sets}
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{lccc}
    \cline{2-4}
         & \multicolumn{3}{c}{\textbf{Evaluation datasets}}\\
         \cline{2-4}
         &  \textit{\makecell{Image \\ Classification}} & \textit{\makecell{Object \\ Detection}}  & \textit{\makecell{Semantic \\ Segmentation}}\\
         \midrule
         RVSA&  \makecell{\textbf{UCM}, \textbf{AID},\\ \textbf{NWPU}}&  \makecell{\textbf{DIOR-R},\\ DOTA-V1.0}& \makecell{\textbf{Potsdam}, \\iSAID, \textbf{LoveDA}}\\[0.4cm]
         RingMo& \makecell{\textbf{UCM}, \textbf{AID},\\ \textbf{NWPU}}&  \makecell{\textbf{DIOR},\\ FAIR-1M}& \makecell{\textbf{Potsdam},\\ iSAID}\\[0.4cm]
         MTP&  \makecell{EuroSAT,\\ \textbf{NWPU}}&  \makecell{ \textbf{DIOR/-R}, FAIR1M,\\ DOTA V1.0/V2.0}& \makecell{SpaceNetv1, \\ \textbf{LoveDA}}\\[0.4cm]
 BFM& -& \makecell{\textbf{DIOR-R},\\ DOTA-V2.0} & \makecell{\textbf{Potsdam},\\ \textbf{LoveDA}}\\
 \midrule
 \textsc{Quetzal-MR} & \makecell{\textbf{UCM}, \textbf{AID},\\ \textbf{NWPU}} & \textbf{DIOR},\textbf{DIOR-R} & \makecell{\textbf{Potsdam},\\ \textbf{LoveDA}} \\
 \bottomrule
    \end{tabular}
\end{table}

% RVSA: UCM, AID, NWPU-RESISC; DOTA-V1.0, DIOR-R; Potsdam, iSAID, LoveDA
% MTP: EuroSAT, NWPU-RESISC; xView, DIOR,DIOR-R, FAIR1M, DOTA-V1.0/V2.0; SpaceNetv1, LoveDA
% RingMo: AID, NWPU-RESIS, UCM; DIOR, FAIR-1M; iSAID, Potsdam
% BFM: ; DIOR-R, DOTA v2.0; Potsdam, LoveDA

By their nature, FMs are very large, such that fine-tuning fewer tasks-specific layers is preferable from the perspective of computational and labeled-data budgets. Fine-tuning configurations can range between updating all layers of the model during downstream specialization, freezing specific layers/blocks (e.g., the pretrained backbone), to the linear probing configuration where all pretrained parameters are frozen and parameter updates are thus restricted only to a final classification layer appended to the pretrained model.

Results are typically contrasted to baselines trained in fully supervised schemes for multiple tasks. 

% \todo[inline]{Discuss challenges for semantic segmentation and object detection using ViT-e (3B). For semantic segmentation, the adopted UperNet configuration with Potsdam HxW and LoveDA HxW image crop-sizes does not fit in a single GPU, requiring still ongoing work of adapting of mmsegmentation or a separate codebase to incorporate model sharding in semantic segmentation setups. Meanwhile, while we are able to fit in a $80GB$ GPU a configuration employing ViT-e (3B) as backbone of a ViTDet for object detection, the finetuning configuration that worked for ViT-Base and ViT-g (1B) did not scale well for such 3B model variant, requiring further studies on optimization dynamics.  }

\subsection{Image classification}
We followed \cite{wang2022rvsa} and \cite{sun2022ringmo} and assessed model downstream capabilities across the UC Merced Land Use (UCM) \cite{Yang2010UCM}, the Aerial Image Dataset (AID) \cite{xia2017aid}, and the NWPU-RESISC45 \cite{cheng2017nwpu} collected by the Northwestern Polytechnical University. Table~\ref{table:datasets} presents an overview of these datasets. 
% Scaling can require different linear rate schedulers than the ones used for base -- discuss having a fixed budget like GeoBench suggests

\begin{table}[h!]
\caption{The different datasets used for linear-probing + evaluation on downstream tasks.}
\centering
\begin{tabular}{ cccc }
 \toprule
   \multicolumn{4}{c}{\textit{Image Classification}} \\
   \midrule
 \textbf{Datasets} & \textbf{Training Samples}  & \textbf{Testing Samples} & \textbf{Classes} \\
 \midrule
%  \multicolumn{4}{|c|}{\textit{Pretraining}} \\
%  \hline
%  MillionAID   & 990848    &  &   \\
%  \hline
%  \multicolumn{4}{|c|}{\textit{Image Classification}} \\
%  \hline
 % MillionAID &   1000  & 9000  & 51 \\
 UCM &   1050  & 1050  & 21 \\
 AID &   2000  & 8000  & 30 \\
 NWPU &   3150  & 28350  & 45 \\
 \bottomrule
%   \hline
%  \multicolumn{4}{|c|}{Semantic Segmentation Dataset} \\
%  \hline
%  LoveDA &   2522  & 1669  & 7 \\
%   \hline
\end{tabular}
\label{table:datasets}
\end{table}

% \begin{table}[h!]
% \centering
% \caption{Linear Probing results across different RS image classification datasets}
% \addtolength{\tabcolsep}{-0.1em}
% \begin{tabular}{ |c|c|c|c|c|c| }
%  \cline{3-6}
%  \multicolumn{2}{c|}{} & \multicolumn{4}{c|}{\textbf{Top1 Acc ($\%$) on}} \\
%  \hline
%  \textbf{Model} & \textbf{\makecell{Pretrain \\ epochs}} & \textbf{\textit{UCM}} & \textbf{\textit{AID}} & \textbf{\textit{NWPU}} & \textbf{\textit{{MillionAID}}} \\
%  \hline
%  MAE-Base\cite{wang2022rvsa}$^\dag$ & 400 & 49.90  & 61.70 & 61.28 & \\
%  MAE-Base & 400 & 45.17 & 52.11 & 54.28 & 47.20 \\
%  MAE-Base & 100 & 40.62 & 41.72 & 42.40 & 41.31 \\
%  MAE-Huge & 100 & 50.00 & 60.78 & 57.24 & 53.28 \\
%  MAE-1B & 100 &  57.10 & 68.89 & 64.35 & 59.14 \\
%  MAE-3B & 100 & 74.05 & 79.96 & 76.43 & 72.98 \\
%  \hline
% \end{tabular}
% \raggedleft
% \footnotesize{$^\dag$results in \cite{wang2022rvsa} are obtained for different data splits as discussed in the text.}\\
% \label{table:results}
% \end{table}

% \begin{figure*}[h!]
% \centering
% \begin{minipage}[t]{1.25\textwidth}
%   \centering
%   \hspace*{-5cm}\includegraphics[width=1.\linewidth]{plots/linprob_test_acc1.png}
% \end{minipage} \hfill
% \begin{minipage}[t]{1.25\textwidth}
%   \centering
%   \hspace*{-5cm}\includegraphics[width=1.\linewidth]{plots/linprob_test_acc5.png}
% \end{minipage}\hfill
% %\begin{subfigure}{1.25\textwidth}
% %  \centering
% %  \hspace*{-5cm}\includegraphics[width=1.\linewidth]{plots/linprob_test_loss.png}
% %\end{subfigure}\hfill
% \caption{The top1 and top5 classification accuracy, of the linear probe classification for the four MAE pretrained ViT models: base, huge, 1B and 3B for all testing datasets. The 100 epochs checkpoint was used from the pretraining, for each model architecture, while keeping all the hyper-parameters constant for the classification task. The training and testing dataset split is as shown in table \ref{table:datasets}}
% \label{fig:lin-prob-all}
% \end{figure*}

Such difference is an indicator that learning rate schedules being used so far in the literature for finetuning in these datasets is suboptimal, not leveraging full model capabilities. 

After the self-supervised pretraining, we used linear probing for downstream adaptation of the MAE-pretrained ViT models for image classification. Following common practice \cite{he2022masked}, the LARS \cite{you2017large} optimizer was used, with a base learning rate of 0.1 and no weight decay. The MLP heads of the model were replaced by a linear classifier for supervised training while keeping the weights for the rest of the model frozen. The hyper-parameters were kept identical for all models and datasets. A total number of 100 epochs was used for all the measurements. The global batch-size for UCM, AID and NWPU was kept identical with \cite{wang2022rvsa} at 256.

We opt for pretraining our models for 100 epochs and fine-tuning for 100 epochs, in contrast to the 400 epochs of pretraining and 200 epochs of fine-tuning adopted for the ViT-Base models reported in \cite{wang2022rvsa}. Rather than pursuing an indiscriminate use of computing resources and energy, we restrict the pretraining of our models as the results obtained already support the hypothesis that significant improvements are obtained as the models are scaled in size. Table \ref{table:results} shows the top1 classification accuracy for the ViT-Base, ViT-Huge, ViT-1B and ViT-3B for all four image classification datasets. 


\begin{table}[h!]
\centering
\caption{Linear Probing results across different RS image classification datasets.}
% \todo[inline]{Perhaps try much lower splits here, to simulate few-shot and since these values in the 90\% are super high}
% \addtolength{\tabcolsep}{-0.4em}
\begin{tabular}{ lcccc}
 \cline{3-5}
 \multicolumn{2}{c}{\textbf{\textsc{RVSA}}} & \multicolumn{3}{c}{\textbf{Top1 Acc ($\%$)}} \\
 \hline
 \textbf{Model} & \textbf{\makecell{Pretrain \\ epochs}} & \textbf{\textit{\makecell{UCM\\(TR=$50\%$)}}} & \textbf{\textit{\makecell{AID\\(TR=$20\%$)}}} & \textbf{\textit{\makecell{NWPU\\(TR=$10\%$)}}} \\
 \hline
 % \makecell{ViT-Base\\\cite{wang2022rvsa}}& 400 & 49.90  & 61.70 & 61.28  \\
  \makecell{ViT-B\\\cite{wang2022rvsa}}& 1500 & 98.58  & 93.84 &  87.20 \\
 \hline
\end{tabular}
\\
\vspace{10pt}
% \addtolength{\tabcolsep}{-0.1em}
\begin{tabular}{ lcccc }
 \cline{3-5}
 \multicolumn{2}{c}{\textbf{\textsc{Quetzal-MR}}} & \multicolumn{3}{c}{\textbf{Top1 Acc ($\%$)}} \\
 \hline
 \textbf{Model} & \textbf{\makecell{Pretrain \\ epochs}} & \textbf{\textit{\makecell{UCM\\(TR=$50\%$)}}} & \textbf{\textit{\makecell{AID\\(TR=$20\%$)}}} & \textbf{\textit{\makecell{NWPU\\(TR=$10\%$)}}} \\
 \hline
 % ViT-Base & 400 & 45.17 & 52.11 & 54.28  \\
 ViT-B & 200 & 97.35  & 93.70 & 86.19 \\
 ViT-H & 200 & 98.39 & 94.76 & 89.73 \\
 ViT-G (1B) & 200 & 94.22 & 89.38  & 79.54 \\
 ViT-e (3B) & 200 & 98.30 & 95.53 & 89.27 \\ 
 % ViT-Base & 100 & 40.62 & 41.72 & 42.40 & 41.31 \\
 % ViT-Huge & 100 & 50.00 & 60.78 & 57.24 & 53.28 \\
 % ViT-1B & 100 &  57.10 & 68.89 & 64.35 & 59.14 \\
 % ViT-3B & 100 & 74.05 & 79.96 & 76.43 & 72.98 \\
 \hline
\end{tabular}
\label{table:results_linprob}
\end{table}


% \begin{figure*}[t]
%     \centering
%      \begin{subfigure}[b]{0.32\linewidth}
%      \centering
%         \includegraphics[width=\linewidth, height=2.5cm]{example-image-a}
%          \caption{image classification (AID)}
%          \label{fig:img-conv}
%      \end{subfigure}    
%      \begin{subfigure}[b]{0.32\linewidth}
%      \centering
%         \includegraphics[width=\linewidth, height=2.5cm]{example-image-b}
%          \caption{semantic segmentation (Potsdam)}
%          \label{fig:sseg-conv}
%      \end{subfigure}    
%      \begin{subfigure}[b]{0.32\linewidth}
%      \centering
%         \includegraphics[width=\linewidth, height=2.5cm]{example-image-c}
%          \caption{object detection (DIOR-R)}
%          \label{fig:objdet-conv}
%      \end{subfigure}  
%      \caption{Convergence curves for finetuning of different pretrained models}    
% \end{figure*}

% We kept the original split that was given from the database we download the data from, and as far as we can tell there is no an established split for those three datasets.

Importantly, results in Table \ref{table:results_linprob} clearly reveal improvements in image classification performance as we scale the model size, for all three datasets evaluated.

% Remarkably, we observe more than $30\%$ improvement across all four datasets when going from a 100M parameter to a 3B parameter model. 

% The differences in performance we observe between the ViT-Base reported in \cite{wang2022rvsa} and ours are most likely due to differences in data splits used for each dataset, as we adopt more rigorous training/test splits (i.e., fewer training samples). We denote TR the ratio of training samples used for each dataset: while we adopt $TR=50\%$ for UCM, $TR=20\%$ for AID and $TR=10\%$ for NWPU, results in \cite{wang2022rvsa} were obtained with $TR=55\%$ for UCM, $TR=17\%$ for AID and $TR=19\%$ for NWPU. Still, the pattern of performance improvement as our models are scaled in size is evident, with results obtained by our ViT-Huge and larger models surpassing these numbers despite relying on fewer training samples and pretraining epochs.

% Figure \ref{fig:lin-prob-all} expands the Table \ref{table:results} by displaying the classification accuracy as a function of the number of linear probing training epochs, for the top1 and top5 classification accuracies. These curves reveal that top1 accuracy improvements become evident even as early as after 10 training epochs for UCM, AID and NWPU datasets, while the top5 accuracy follows a slower trend of improvement. In contrast, it is interesting to note how improvements for the MillionAID dataset occur rather later during training. Since MillionAID samples were also used for pretraining, the linear probing training samples in this case come from the same data-distribution as the pretraining samples. We conjecture this is the main factor explaining this difference with respect to the behavior observed for the other three datasets. }

\subsection{Object detection}
% \todo[inline]{Jordan/Lexie: Description similar to MTP paper, including: dataset description; object detection head used; mmdetection/mmrotate; hyperparameters etc}

For object  detection, we selected DIOR and DIOR-R as the datasets for evaluating downstream tasks. \textit{DIOR} is a remote sensing dataset introduced by Li et al. as an object detection benchmark \cite{Li_2020}. The dataset has 23,463 800x800-pixel RGB images sourced from Google Earth. The images have ground sample distances of 0.5m to 30m. There are 20 object classes and a total of 192,472 object instances. DIOR is divided into training, validation, and testing sets with 5,862, 5,863, and 11,738 images, respectively. As in \cite{wang2024mtp}, we use the training and validation sets in a combined 11,725-image "trainval" set for fine-tuning, and we validate using the testing set. \textit{DIOR-R} is a version of DIOR with oriented bounding box annotations \cite{Cheng_2022}. The images, object classes, object instances, and data splits are identical to DIOR.

%\paragraph{FAIR1M}
%FAIR1M is an oriented object detection dataset containing images sourced from Gaofen satellites and Google Earth \cite{sun2021fair1m}.

% Fine-grAined object recognItion in high-Resolution remote sensing imagery (FAIR1M)

We used the pretrained ViT weights for VitDet \cite{li2022exploring}, a ViT-based object detection architecture that demonstrates promising performance with minimal adaptation of backbones required. Faster-RCNN \cite{7410526} was used as the detection head for the horizontal object detection task, and its variant oriented  Faster-RCNN was used for the oriented object detection task. The VitDet implementation was based on mmdetection \cite{mmdetection} for DIOR data, and the same implementation was further adapted for DIOR-R data using the mmrotate \cite{zhou2022mmrotate} library. Both libraries were also used during fine-tuning and evaluation, which is based on Mean Average Precision (mAP) calculated at Intersection over Union (IoU) threshold 50\%.

As in \cite{li2022exploring}, we adopt a patch size of 16 for all ViT backbones and we interpolate the patch embedding filters for the ViT-H and ViT-1B backbones which used a patch size of 14 during pretraining. With the pretrained ViT weights, we finetuned on DIOR and DIOR-R for 12 epochs, the same as the setting in \cite{wang2024mtp}. The initial learning rate was 3e-4, and the batch size was 4. Training followed a multi-step learning rate schedule with a 500-iteration warmup period, a gamma of 0.1, and learning rate decay at 8 and 11 epochs. A layer-wise learning rate decay of 0.9 was used.

For DIOR, we first can see that Quetzal-MR with ViT-B yields better results than SatMae, ScaleMAE results, which are pretrained on fMoW data. While differences in backbone, the better performance from our ViT-B model can be seen compared to RingMo (ISSP), which utilized the ImageNet Data for pre-training.   The results of DIOR-R, listed in Table \ref{tab:objdet}, reveal that our pretrained model again outperforms those derived from fMoW (SatMae, ScaleMAE). This may be attributed to the larger dataset included in Quetzal-MR.  Furthermore, although the detection head differ slightly, our results excel against MAE ViT-B (66.65\% with oriented RCNN vs. 68.58\% oriented faster RCNN), which also uses the MillionAid dataset. It's also worth noting that we also trained our  pretrained models for fewer epochs compared to fMoW-based and MillionAid-based models while obtained better results as shown in Table \ref{tab:pretrain_datasets}. 

Our ViT-B yields results comparable to BFM (68.58\% v.s. 68.52\%). Notably, we used a vanilla oriented-faster RCNN for these experiments, while BFM used more advanced ROI transformers on top of oriented-faster RCNN detection head. We also observed that the advantage of using ROI transformer as the detection head becomes more significant as the model size scales. When comparing our vanilla ViDET + oriented faster RCNN results with ViT-B to ViT-G, the improvements from parameter scaling hover around 2.8\%, which is less than the BFM counterpart (~5\%). In general, the scaling benefits in model sizes (ViT-B, ViT-H, and ViT-G) is clear for both datasets. We also discovered the necessities to adjust LRs when scaling model sizes for fine-tuning to obtained better results, particularly for the DIOR-R dataset. We suspect that when going with larger models, the learning decay policy could be more complicated and requires more considerations.

\begin{table}[h]
\centering
\setlength{\tabcolsep}{3pt}
\begin{threeparttable}
  \caption{Summary of results for object detection benchmarks.}
  \label{tab:objdet}
  \begin{tabular}{llcc}
    \toprule
    \textbf{Method} & \textbf{Backbone} & \textbf{\makecell{DIOR \\{} [mAP$_{50}$]}} & \textbf{\makecell{DIOR-R \\{} [mAP$_{50}$]}} \\
    \midrule
    GASSL \tnote{1} & ResNet-50 & 67.40 \cite{wang2024mtp} & 65.65 \\
    MAE \cite{wang2022rvsa} & ViT-B & - & 66.65  \\
    % MAE \cite{wang2022rvsa} & ViTAE-B & - & 68.40 & \\
    RVSA (MAE) \cite{wang2024mtp} & ViT-B + RVSA & 75.80 \cite{wang2024mtp} & 70.85 \cite{wang2022rvsa} \\ 
    % MAE \cite{RVSA} & ViTAE-B + RVSA & - & 71.05 & \\
    MTP \cite{wang2024mtp} & ViT-B + RVSA & 79.40 & \\
    RVSA (MAE) \cite{wang2024mtp} & ViT-L + RVSA & 78.30 & \\ 
    MTP \cite{wang2024mtp} & ViT-L + RVSA & 81.10 & \\    
    SatMAE \tnote{1}& ViT-L & 70.89 \cite{Guo2023SkySenseAM} & 65.66 \cite{Guo2023SkySenseAM} \\
    GFM \tnote{1}\cite{mendieta2023towards} & Swin-B & 72.84 \cite{wang2024mtp} & 67.67 \cite{Guo2023SkySenseAM} \\
    ScaleMAE \tnote{1}& Swin-B & 73.81 \cite{wang2024mtp} & 66.47 \cite{Guo2023SkySenseAM} \\
    RingMo (ISSP) \tnote{2} \cite{sun2022ringmo}& Swin-B & 73.50 & \\
    RingMo \cite{sun2022ringmo}& Swin-B & 75.90 & -  \\
    BFM \cite{cha2023billion} & ViT-B & - & 68.52 \\
    BFM \cite{cha2023billion} & ViT-L12$\times4$ (605M) & - & 72.11  \\
    BFM \cite{cha2023billion} & ViT-H12$\times4$ (1.36B) & - & 73.15  \\
    BFM \cite{cha2023billion} & ViT-G12$\times4$ (2.42B) & - & 73.62  \\
    \midrule
    SkySense & Swin-L & 76.74 & - \\
    SkySense & Swin-H & 78.73 & - \\
    \midrule
    \textsc{Quetzal-MR} & ViT-B & 75.50 & 68.58 \\
    \textsc{Quetzal-MR} & ViT-H & (pretraining) & \\
    \textsc{Quetzal-MR} & ViT-G (1B) & 77.40 & 71.31 \\
    % \textsc{Quetzal-MR} & ViT-e (3B) & Failed & Failed \\
  \bottomrule
\end{tabular}
% \begin{tablenotes}\footnotesize
\begin{tablenotes}[flushleft]\footnotesize
    \item [1]Since GASSL, SatMAE, ScaleMAE and GFM did not provide evaluation on DIOR and DIOR-R in their original papers, we rely on results provided in \cite{wang2022rvsa,wang2024mtp} for each corresponding method as indicated by the citations accompanying each number.    
% \end{tablenotes}
 \item[2] ISSP indicates the RinMo FM was obtained with ImageNet data using a self-supervised pretraining strategy \cite{sun2022ringmo}. 
\end{tablenotes}
\end{threeparttable}
\end{table}
% \todo[inline]{placeholder for sample size analysis associated with Figure 3/4.}
\subsection{Semantic segmentation}
% - For each dataset, have table and curves. Curves show early convergence, benefit of pretraining 
% - Curves using percentages of labeled dataset (e.g., $1\%$, $10\%$, $50\%$)
% - on experiments with data percentage, discuss how works do not describe whether they use the same amount of effective iterations. 


We conduct semantic segmentation experiments with the Potsdam and LoveDA described below. In addition to finetuning configurations where all model parameters are updated, to assess the quality of features learned during pretraining we follow evaluation practices from the broader literature on foundation models and evaluate tuning the model with frozen backbone, as well as varying the percentage of training samples available for finetuning.

\noindent\textbf{Datasets} \paragraph{LoveDA} The LoveDA dataset\cite{wang2021loveda} comprises of 5987 high resolution imagery from Google Earth, acquired at a spatial resolution of \textit{0.3m}. Encompassing both urban and rural landscapes over the cities of Nanjing, Changzhou and Wuhan in China, the dataset consists of per-pixel annotations across 7 land cover classes - \textit{building, road, water, barren land, forest, agriculture and background.} The dataset consists of 1024 X 1024 sized image patches with the training, validation and test sets comprising of 2522, 1669 and 1796 patches respectively. The evaluation metrics for experiments with LoveDA have been computed on the test set using the evaluation server.
%1024X1024
%val files = 1669
%train files = 2522
%test files = 1796

\paragraph{ISPRS Potsdam}
The ISPRS Potsdam dataset from ISPRS WG III/4 (2012-2016) and WG II/4 (2016-2022), consists of 38 tiles of high-resolution orthoimagery captured over the city of Potsdam, Germany, with a spatial resolution of \textit{0.5m}. The dataset has been manually annotated into 6 land cover classes - \textit{impervious surfaces, building, low vegetation, tree, car and clutter/background.} The images are tiled into 512 X 512 sized patches with the training set and test set comprising of 3456 and 2016 patches respectively.
%512X512
%val files = 2016
%train files = 3456

Following common practice across related works \cite{wang2022empirical, sun2022ringmo, Guo2023SkySenseAM}, we adopt the UperNet  scheme \cite{xiao2018upernet} to compose segmentation frameworks for all our considered pretrained backbones.


% \begin{figure}
%     \centering
%      \begin{subfigure}[b]{0.9\linewidth}
%      \centering
%         \includegraphics[width=\linewidth, height=2.5cm]{example-image-a}
%          \caption{semantic segmentation (Potsdam)\todo[inline]{Abhishek/Jordan: generate this curve, similar to MTP's Fig.3 -- work together}}
%          \label{fig:sseg-dataperc}
%      \end{subfigure}    
%     \begin{subfigure}[b]{0.9\linewidth}
%      \centering
%         \includegraphics[width=\linewidth, height=2.5cm]{example-image-b}
%         \caption{object detection experiments (DIOR-R)\todo[inline]{Jordan: generate this curve, similar to MTP's Fig.3}}
%         \label{fig:objdet-dataperc}
%     \end{subfigure}    
%     \caption{Finetuning accuracy of different pretrained models with varying training set sizes.}   
% \end{figure}

\begin{table}
  \caption{Summary of results for semantic segmentation benchmarks.}
  \setlength{\tabcolsep}{3.pt}
  \label{tab:semseg}
  \begin{threeparttable}  
  \begin{tabular}{llcc}
    \toprule
    \textbf{Method} & \textbf{Backbone} & \textbf{\makecell{Potsdam \\{}[mF1 $\%$]}} & \textbf{\makecell{LoveDA \\{}[mIoU $\%$]}} \\
    \midrule
    GASSL \cite{ayush2021geography} & ResNet-50 & 91.27 \cite{Guo2023SkySenseAM} & 48.76 \cite{wang2024mtp}\\
    MAE \cite{wang2022rvsa} & ViT-B & 90.32 & 51.09\\
    % MAE \cite{wang2022rvsa} & ViTAE-B & 91.05 & 52.58 \\
    RVSA (MAE) \cite{wang2022rvsa} & ViT-B + RVSA & 90.77 & 51.95\\
    % MAE \cite{wang2022rvsa} & ViTAE-B + RVSA & 91.15 & 52.44\\
    MTP \cite{wang2024mtp} & ViT-B + RVSA & - & 52.39\\
    RVSA (MAE) \cite{wang2022rvsa} & ViT-L + RVSA & - & 53.72\\
    MTP \cite{wang2024mtp} & ViT-L + RVSA & - & 54.17\\    
    SatMAE \cite{cong2022satmae} & ViT-L & 90.63 \cite{Guo2023SkySenseAM} & -\\
    ScaleMAE \cite{reed2023scalemae} & ViT-L & 91.54 \cite{Guo2023SkySenseAM} & -\\
    GFM \cite{mendieta2023towards} & Swin-B & 91.85 \cite{Guo2023SkySenseAM} & -\\
    RingMo (ISSP) \cite{sun2022ringmo} & Swin-B & 91.27 & - \\
    RingMo \cite{sun2022ringmo} & Swin-B & 91.74 & - \\
    BFM \cite{cha2023billion}& ViT-L12$\times4$ (605M) & 91.75 & 52.38 \\
    BFM \cite{cha2023billion}& ViT-H12$\times4$ (1.36B) & 92.02 & 53.20 \\
    BFM \cite{cha2023billion}& ViT-G12$\times4$ (2.42B) & 92.12 & 54.40 \\
    \midrule
    SkySense \cite{Guo2023SkySenseAM} & Swin-L & 92.86 & -\\
    SkySense \cite{Guo2023SkySenseAM} & Swin-H & 93.99 & -\\
    \midrule
    \textsc{MAE\tnote{$\diamondsuit$}} & ViT-B & 91.82 & - \\
    \textsc{Quetzal-MR} & ViT-B & 92.01 & 52.44 \\
    \textsc{Quetzal-MR} & ViT-H & 92.18 & 53.83 \\
    \textsc{Quetzal-MR} & ViT-G (1B) & 92.20 & 54.00 \\
    % \textsc{Quetzal-MR} & ViT-e (3B) & (remove?) & \\
    % MAE & ViT-e (3B) & &\\
  \bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]\footnotesize
    \item[$\diamondsuit$] Pairing pretrained weights from \cite{wang2022rvsa} with our finetuning parameterization.
    \item Since GASSL, SatMAE, ScaleMAE and GFM did not provide evaluation on Potsdam and LoveDA in their original papers, we rely on results provided in \cite{wang2022rvsa,wang2024mtp} for each corresponding method as indicated by the citations accompanying each number.
\end{tablenotes}
\end{threeparttable}
\end{table}
\begin{table}
  \caption{Results for finetuning with frozen backbone (Frozen/Not-Frozen)}
  \label{tab:frozen}
  \begin{tabular}{llcc}
    \toprule
    \textbf{Method} & \textbf{Backbone} & \textbf{\makecell{Potsdam \\{}[mF1$\%$]}} & \textbf{\makecell{DIOR-R \\{}[mAP$\%$]}}  \\
    \midrule
    \textsc{Quetzal-MR} & ViT-B & 88.97/92.01 & 68.33/68.58 \\ %3e-4: 67.04/66.52 frozen/non-frozen
    \textsc{Quetzal-MR} & ViT-H & 89.75/92.18 & / \\
    \textsc{Quetzal-MR} & ViT-G (1B) & 89.62/92.20 & 71.06/71.31\\
    % \textsc{Quetzal-MR} & ViT-e (3B) & R/R & R/R \\
  \bottomrule
\end{tabular}
\end{table}

\noindent\textbf{Implementation details.} All experiments are implemented using the \textit{mmsegmentation} codebase. Following \cite{wang2022empirical, wang2022rvsa}, we configured the UperNet architectures with a Feature2Pyramid neck operating with $[4, 2, 1, 0.5]$ rescaling factors. For ViT-B configurations, features are collected from blocks $[3, 5, 7, 11]$ (index starting at 0) of the $12-$layer deep backbone. Since the ViT-H and ViT-g(1B) variants are $32-$ layers deep, we instead collect features from blocks $[11, 17, 23, 31]$. Moreover, a FCN with $256$ channels and loss weight of $0.4$ as auxiliary head.

Configurations reported in \cite{wang2022rvsa} and \cite{cha2023billion} employ $160k$ iterations at batch size $8$, base LR of $6e-5$ and weight decay of $0.01$ for Potsdam and LoveDA, while \cite{sun2022ringmo} and \cite{Guo2023SkySenseAM} adopt $80k$ iterations for the same set of hyperparameters on Potsdam. This corresponds to finetuning durations of $1.28M$ and $0.64M$ iterations at batch-size $1$. To efficiently evaluate different model sizes across several configurations (i.e., frozen backbone and different training data percentages), we conduct these experiments under a distributed computing setup where such a small batch size is sub-optimal. Following experimentation with base learning rates for ViT-B on Potsdam, for all our semantic segmentation experiments we adopt an effective batch-size of $256$, with a base learning rate of $5e-4$ paired with CosineAnnealingLR scheduled with $50$ epochs of warmup and finetuning duration of $100$ epochs for each dataset. This corresponds to $345.6k$ iterations (at batch size $1$) for Potsdam and $419.1k$ iterations for LoveDA, which is equivalent to only $27\%$ of the iterations reported by \cite{wang2022rvsa, cha2023billion} for Potsdam and $65.5\%$ of the duration reported in \cite{wang2022rvsa} for LoveDA.

\noindent\textbf{Experimental results.} Table \ref{tab:semseg} summarizes results of our \textsc{Quetzal-MR} model variants in contrast to related works on the Potsdam and LoveDA datasets. Most importantly, we observe significant benefits of model scaling. This is particularly evident for results on LoveDA, where scaling from ViT-B (89M) to ViTG (1B) provides an improvement of $+1.56\%$ in test mIoU. In contrast to metrics reported by previous works, it is noteworthy how our ViT-B configuration outperforms by $+1.69\%$ in Potsdam and $+1.35\%$ the results reported in \cite{wang2022rvsa} for a MAE similarly pretrained using MillionAID, but for twice the number of pretraining epochs. Similarly, we also note how metrics of our 1B model variant are on par with results reported for BFM's 2.4B model variant \cite{cha2023billion}. In addition to indicating the good quality of our pretraining and finetuning setups, such differences are indicators that learning rate schedules being used so far in the literature for finetuning in these datasets is suboptimal, not leveraging full model capabilities. 

Table \ref{tab:frozen} further provides results contrasting aforementioned finetuning results with configurations

\section{\textsc{Quetzal-HR} experiments}
We leverage the building footprint labels available as part of the ORBITaL-Net dataset for evaluation of our \textsc{Quetzal-HR} model variants. 

\noindent\textbf{Dataset and experimental scenarios.} Two finetuning configurations were considered for building footprint extraction (BFE) tasks: \textit{$TR=100\%$}, where finetuning takes place for $100$ epochs using $55.71k$ training labeled tiles (i.e., $5.57M$ iterations); \textit{$TR=10\%$}, where we use instead a randomly sampled subset with $5571$ ($10\%$) tiles for finetuning for $100$ epochs (i.e., $557.1k$ iterations). For both cases, evaluation takes place using a separate validation set of $4836$ tiles from the ORBITaL-Net dataset. The rationale behind these configurations is that \textit{$TR=100\%$} provides an upperbound of performance achievable by training/finetuning with a fully labeled dataset for a large number of iterations. Meanwhile, results with the \textit{$TR=10\%$} configuration assess FM capabilities by measuring how close to this upperbound a corresponding pretrained model is able to perform when finetuned using significantly fewer labeled samples and finetuning iterations.

\noindent\textbf{Implementation details}: similar to experiments reported in section \ref{sec:experiments_mr}, UperNet is paired to pretrained \textsc{Quetzal-HR} variants for semantic segmentation. Feature pyramids and rescaling factors are the same as reported in section \ref{sec:experiments_mr}, with the auxiliary FCN head however removed to reduce computing workload. Experiments are performed with a effective batch size of $2048$, AdamW with betas (0.9, 0.999), base learning rate of $1e-3$, and a cosine annealing LR schedule with $10$ epochs of warmup. Image size of $512\times512$ is adopted for Vit-B configurations and $504\times504$ for larger configurations trained with patches $14\times14px$ large, to bypass mmsegmentation errors related to non-integer number of patches.
% UperNet (no auxiliary head), LR=1e-3, BS=16*8*16, LayerDecay with decay rate of 0.9, AdamW with betas (0.9, 0.999) and WD=0.05, 100 epochs, 10 epochs of warmup, cosine annealing OneCycleLR, imgsize=512/504, random crop (ratio 0.5-2.0), random flip*. Note on how the \textit{outindices} are selected as models are scaled

% As such, this indicates that the $TR=10\%$ configuration is more suitable to assess performances of a FM, as their main goal is to adapt to downstream tasks using as few labeled samples and finetuning iterations as possible. Thus, 


% \textit{Implementation details} detail a bit more the FT with topo-loss, effective batch size etc

In the paragraphs below, we discuss the multiple takeaways that can be extract from the results summarized in Table \ref{tab:bfe_semseg}.


\begin{table}[h]
  \caption{Summary of results enabled by \textsc{Quetzal-HR} model variants for semantic segmentation on ORBiTal-Net dataset.}
    % \setlength{\tabcolsep}{3pt}
  \label{tab:bfe_semseg}
  \begin{threeparttable}
    \begin{tabular}{lllcc}
    \toprule
    \textbf{Method} & \textbf{Backbone} & \textbf{\makecell{Pretrain \\ dataset}} & \multicolumn{2}{c}{\bfseries BFE - mF1[\%]}\\ \cline{4-5}
    & &  &  $TR=100\%$ & $TR=10\%$  \\
    \midrule
    No pretrain & ViT-B & - & 91.80 & 74.68 \\
    \midrule
    MAE & ViT-B & ORB & 91.79 & 89.57\\ %90.88 (test)
    MAE & ViT-H & ORB & 91.31 & 88.59 \\ %90.49
    \midrule
    MAE & ViT-B & TIU & 92.05 & 89.85\\ %90.99 
    MAE & ViT-H & TIU & 92.54 & 91.13 \\ %91.53    
    % MAE & ViT-G$_{224}$ & TIU & & \\ %91.53
    % MAE & ViT-G (1B) & TIU & \\ % pretraining ongoing 
    \midrule
    \makecell[l]{\textsc{Q-MR}\tnote{1} \\ + MAE} & ViT-B & TIU & 92.15 & 90.17 \\% pretraining ongoing
    \midrule
    MAE & ViT-B & TIU+ORB & 91.94 & 90.07\\ %90.99 
    % MAE & ViT-H$_{224}$ & TIU+ORB & PT &  \\ %91.53
    MAE & ViT-H & TIU+ORB & 92.84 & 91.70 \\ %91.53    
    MAE & ViT-H$_{224}$ & TIU+ORB & - & 90.38 \\ 
    % MAE & ViT-G (1B) & TIU+ORB & PT & \\ % pretraining ongoing 
    % MAE (inflated) & ViT-H & TIU & (pretraining) & \\% pretraining ongoing
    % MAE (inflated) & ViT-G (1B) & TIU & & \\% TBD based on Base and H  
  \bottomrule
\end{tabular}
\begin{tablenotes}\footnotesize
    \item[1] model initialized with \textsc{Quetzal-MR} (RGB) weights pretrained on MillionAID and then inflated to 4-bands.
\end{tablenotes}
\end{threeparttable}
\end{table}


\noindent\paragraph{Pretraining on ORB dataset vs no pretrain} While the performances of a ViT-B trained from scratch and a model pretrained on ORB and then finetuned as per the $TR=100\%$ configuration are nearly equal, contrasting the F1 numbers obtained in the $TR=10\%$ regime using fewer labeled samples and finetuned for fewer iterations does reveal a significant benefit of pretraining. Thus, while MAE pretraining on a dataset containing the same samples used for finetuning does not improve F1 rates when the supervised learning occurs for a long computing and labeling budget, it does provide benefits in terms of convergence to solution at a lower computing/labeling budget.

\noindent\paragraph{Model scaling requires data scaling, and larger models benefit more from data scaling} Performances obtained by ViT-H model variations pretrained on the ORB dataset are worse than ViT-B for both finetuning configurations ($-0.48/-0.98\%$). In contrast, pretraining with the larger and diverse TIU dataset enables a ViT-H model to significantly outperform ViT-B counterparts in both finetuning configurations ($+0.49/+1.28$). The higher model capacity of ViT-H enables better leveraging the TIU dataset to improve overall segmentation quality, with an increase in F1 of $+0.74\%$ with respect to ViT-B trained from scratch under $TR=100\%$ as compared to the $+0.25\%$ observed for ViT-B pretrained configuration. Compared to their ViT-B counterparts ($-0.11/+0.22\%$), the ViT-H configurations also benefit more from pretraining on the larger TIU+ORB dataset ($+0.30/+0.57\%$) as compared to pretraining on TIU only. This is particularly evident for the $TR=10\%$ configuration, reaching F1 numbers similar to the ones obtained by ViT-B configurations fine-tuned using the $TR=100\%$ finetuning budget. Figure \ref{fig:bfe} provides a qualitative example of the improvements provided by a ViT-H pretrained in TIU compared to outputs from the ViT-B pretrained on ORB.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/ex_BFE_placeholder.png}
    \caption{Qualitative example comparing BFE outputs by a ViT-H pretrained in TIU (in blue) compared to a ViT-B pretrained on ORB only (in pink). ViT-H outputs improve adherence to building boundaries in both exampels, and retrieving better delineations including in areas of low image contrast (e.g., lower-left building in left-most example).}
    \label{fig:bfe}
\end{figure}


\noindent\paragraph{Initialization using inflated \textsc{Quetzal-MR} weights.} In addition to pretraining using BGR+NIR high-resolution optical imagery, we considered whether the RGB-only MillionAID dataset could also be leveraged to further benefit the development of our 4-band \textsc{Quetzal-HR} model variants. To that end, we considered an additional configuration where, prior to MAE pretraining using our TIU dataset, we initialized a ViT-B by inflating the 3-band (RGB) \textsc{Quetzal-MR} pretrained weights with randomly initialized weights associated to a 4th-band. The intuition behind this design is that the \textsc{Quetzal-MR}'s weights pretrained on MillionAID would offer a strong initialization for feature extraction from the RGB bands, leading to two potential benefits: i) speed up pretraining convergence; ii) improve overall feature extraction capabilities, as the intrinsic earlier exposure of the model to MillionAID's diverse gallery of images could provide indirect data scaling benefits. Results in Table \ref{tab:bfe_semseg} corroborate this idea, as the model obtained through this configuration further boosted the ViT-B F1 rates for both TR finetuning settings by $+0.10/+0.32\%$ in comparison to pretraining on TIU alone. 
% \todo[inline]{include loss curves}

\noindent\paragraph{Pretraining using larger image sizes} Pretraining larger models with smaller patch sizes is a common practice in the literature to reduce computational costs. We investigated the impact of pretraining our ViT-H \textit{Quetzal-HR} model variant using an image size of $224\times224px$ instead of $512\times512$. We refer to this variant as ViT-H$_{224}$. From the perspective of memory footprint, ViT-H$_{224}$ requires 24GB for a batch-size of 64 samples per GPU, in contrast to the 50GB required by the $512\times512px$ counterpart for a batch-size of 16. Finetuning results show that this $>4\times$ reduction in pretraining costs (i.e., number of GPU hours) comes at a cost of dropping $-1.32\%$ in segmentation F1 for BFE in the $TR=10\%$ finetuning regime. This indicates that, if computing budget can be afforded, pretraining a high-resolution model with larger image sizes can significantly benefit downstream tasks that require fine-grained, pixel-level accuracy.

% \noindent\paragraph{Finetuning using larger image sizes} 
% TIU+ORB -> 256: 86.13; 512: 90.07; 768: 91.01

